Solving Linux Upgradeability Problems Using Boolean Optimization

Managing the software complexity of package-based systems can be regarded as one of the main challenges in software architectures. Upgrades are required on a short time basis and systems are expected to be reliable and consistent after that. For each package in the system, a set of dependencies and a set of conflicts have to be taken into account. Although this problem is computationally hard to solve, efficient tools are required. In the best scenario, the solutions provided should also be optimal in order to better fulfill users requirements and expectations. This paper describes two different tools, both based on Boolean satisfiability (SAT), for solving Linux upgradeability problems. The problem instances used in the evaluation of these tools were mainly obtained from real environments, and are subject to two different lexicographic optimization criteria. The developed tools can provide optimal solutions for many of the instances, but a few challenges remain. Moreover, it is our understanding that this problem has many similarities with other configuration problems, and therefore the same techniques can be used in other domains.

==> eptcsdata.tex <==
\providecommand{\event}{I. Lynce and R. Treinen (eds.): Workshop on\\
Logics for Component Configuration (LoCoCo 2010)}
\providecommand{\volume}{29}
\providecommand{\anno}{2010}
\providecommand{\firstpage}{11}
\providecommand{\eid}{2}
\providecommand{\publicationstatus}{I. Lynce and R. Treinen (eds.): Workshop on\\
Logics for Component Configuration (LoCoCo 2010)\\
EPTCS 29, 2010, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.29.2}{10.4204/EPTCS.29.2}}

